OmniLytics+: A Secure, Efficient, and Affordable Blockchain Data Market for Machine Learning through Off-Chain Processing

The rapid development of large machine learning (ML) models requires a massive amount of training data, resulting in booming demands of data sharing and trading through data markets. Traditional centralized data markets suffer from low level of security, and emerging decentralized platforms are faced with efficiency and privacy challenges. In this paper, we propose OmniLytics+, the first decentralized data market, built upon blockchain and smart contract technologies, to simultaneously achieve 1) data (resp., model) privacy for the data (resp. model) owner; 2) robustness against malicious data owners; 3) efficient data validation and aggregation. Specifically, adopting the zero-knowledge (ZK) rollup paradigm, OmniLytics+ proposes to secret share encrypted local gradients, computed from the encrypted global model, with a set of untrusted off-chain servers, who collaboratively generate a ZK proof on the validity of the gradient. In this way, the storage and processing overheads are securely offloaded from blockchain verifiers, significantly improving the privacy, efficiency, and affordability over existing rollup solutions. We implement the proposed OmniLytics+ data market as an Ethereum smart contract [41]. Extensive experiments demonstrate the effectiveness of OmniLytics+ in training large ML models in presence of malicious data owner, and the substantial advantages of OmniLytics+ in gas cost and execution time over baselines.

==> Implementation.tex <==
\section{Implementation}

We implement our proposed \scheme as an Ethereum smart contract \ethcontract, with 400 lines of Solidity code. We deploy the contract on our local Geth Ethereum Testnet~\cite{geth} by Remix IDE~\cite{Remix} and ganache~\cite{ganache}, in which all servers and \drs are assigned unique Ethereum addresses. We implement the \drs and off-chain servers using Go and C++ NTL library\cite{libntl}, enabling multiple \drs and servers to operate on a local machine. We quantize the gradient values onto the finite field \( \mathbb{F}_{2^{127}-1} \). For our implementation of ZK rollups, we utilize the zokrates library~\cite{zokrates} to produce Groth'16 zero-knowledge proofs, preserving the transaction data. The rollup operator aggregates these transactions, and creates a zk-SNARK proof for validation, and then submits this proof alongside a condensed version of the transactions to the Ethereum blockchain.

\noindent \textbf{Machine learning and on-chain interaction.}
We implement the model training on the \mr and the \drs using Python and Pytorch~\cite{pytorch}. We utilize Web3py library~\cite{Web3py} to connect the off-chain parts and the smart contracts. We used single local ethereum address 

\noindent \textbf{Gradient validation circuit.} We adopt the norm threshold test as the validation method for gradients, i.e., $\texttt{Valid}(\vct{g}) = \mathbbm{1}[||\vct{g}||_2 \leq \rho]$, for some threshold $\rho$ provided by the \mr.
% In Step 3: Private gradient validation, the \contract contract reveals the arithmetic circuit for evaluating the $\texttt{Valid}(\cdot)$ predicate provided by the \mr. Specifically, we use Norm Bound to check whether the $\ell_{2^{-}}$-norm of a client update is bounded.  norm of a client update is bounded: $\operatorname{Valid} (u)=\mathbb{I}\left[\|u\|_2<\rho\right]$ where $\mathbb{I}[\cdot]$ is the indicator function and the threshold $\rho$ is computed from the public dataset $\mathcal{D}_P$.
% Since the equality operator $=$ is relatively complicated to implement in an arithmetic circuit, we replace the validation check of the form $\Phi(u)=c_1 \vee \Phi(u)=c_2 \vee \cdots \vee \Phi(u)=c_k$ in the output nodes of Valid(-), where $\Phi(\cdot)$ is some arithmetic function, by an output of the form $\left(\Phi(u)-c_1\right) \times \cdots \times\left(\Phi(u)-c_k\right)$. For a given bound $\rho]$, if the final output of this circuit is 0, the input gradients are deemed valid; otherwise, they are considered invalid.

In Step 3, the contract reveals the arithmetic circuit for evaluating the $\texttt{Valid}(\cdot)$ predicate provided by the MO. Considering the complexity of implementing the equality operator $=$ in arithmetic circuits, we substitute the validation check of the form $\Phi(u) = c_1 \vee \Phi(u) = c_2 \vee \ldots \vee \Phi(u) = c_k$ in the output nodes of Valid(-) with $\left(\Phi(u)-c_1\right) \times \ldots \times \left(\Phi(u)-c_k\right)$. Specifically, for the purpose of validating the gradients, our circuit design employs the formula: $\left( \sum_{i=1}^{n} x_i^2 - 1 \right) \times (x-2) \times \ldots \times (x-p)$ to determine if the result is zero. If it is zero, this indicates that the sum of the squares of the numbers, i.e., $x_1^2 + \ldots + x_n^2$, is less than $p$. We use the norm threshold test as the validation method for gradients, denoted by $\texttt{Valid}(\bm{g}) = \mathbbm{1}\left[ \lVert \bm{g} \rVert_2 \leq \rho \right]$, where the threshold $\rho$ is derived from the public dataset $\mathcal{D}_P$. 



We compare \scheme against total on-chain scheme of the data market.

==> current_solution.tex <==
\section{Summary of Current Solution}

\begin{enumerate}[leftmargin=*]
    \item {\bf Byzantine \mr:} Design the entire data market as a smart contract. This partially solves the problem of Byzantine \mr. \songze{We may need a mechanism to decide on the fair revenue for each \dr (Shapley value?).}
    \item {\bf Model privacy:} Use the model perturbation method in~\cite{yang2020computation}. \songze{Some limitations: 1) only works with mean-square loss; 2) only works for MLP with ReLU activation.}
    \item  {\bf Byzantine \drs:} Use multi-Krum~\cite{blanchard2017machine,blanchard2017byzantine} across \dr groups. \songze{Can we do it with ZK proofs? How about proof of learning~\cite{jia2021proof}?}
    \item {\bf Data privacy:} Use secure aggregation from~\cite{bonawitz2017practical}. Partition \drs into $G$ groups and carry out secure aggregation within each group. \songze{Functional encryption? Efficiency?}
    \item \songze{Now all the above operations are performed on-chain using smart contract, which bring heavy storage and computation complexities, and high gas cost. Can we design an off-chain solution using rollups?}
    

The proposed protocol:
\begin{itemize}
    \item Step 1: The \mr encrypts the initial model using model perturbation~\cite{yang2020computation}. It then publishes the encrypted model, together with the model reward on a smart contract.
    
    \item Step 2: The interested \drs register with the contract. All interested \drs are partitioned into $G$ groups. %each group is assigned a set of secret keys, like in Agora~\cite{koutsos2021agora}.
    
    \item Step 3: \drs train local models with the encrypted model and local data, encrypt the obtained models with secret keys, and upload to contract.
    
    \item Step 4: Contract performs secure aggregation within each group, and outlier removal across groups. These are all done off-chain using rollups. (Can we also move storage off-chain?)
    
    \item Step 5: Contract outputs the aggregation results from the surviving groups. The \mr decrypts the aggregated models with secret key for model perturbation.  
\end{itemize}    
    
    
\end{enumerate}

==> introduction_old.tex <==
\section{Introduction}
With the rapid development of sensing, processing, and storage capabilities of computing devices (e.g., smartphones and IoT devices), the collection and storage of data has been increasingly convenient and cost-effective~\cite{sheng2013sensing,cornet2018systematic}. On the other hand, crowdsourcing big data has been shown to be extremely effective in improving the performance of various tasks in, e.g., healthcare, smart city, and recommender systems~\cite{raghupathi2014big,wang2018big,hashem2016role,al2015applications,yin2013lcars}. The abundant supply of data stored locally at individual nodes and the huge demands from data-intensive applications incentivise the development of a data market, on which data owners can easily trade the rights of using their data with interested consumers for monetary returns.

Conventionally, a data market is often implemented as a centralized service platform that collects data from data owners and sells raw or processed data to the consumers~\cite{mivsura2016data,krishnamachari2018i3,niu2018achieving}. This approach leaves the platform as a single point of security vulnerability for the data market, and corruption on the platform servers may lead to severe security issues including leakage of private data, faulty computation results, and manipulation of data price. A number of recent works have proposed to leverage technologies of decentralized systems like blockchains and smart contracts to tackle the weakness of the centralized implementation (see, e.g.,~\cite{ozyilmaz2018idmob,duan2019aggregating,ramachandran2018towards,koutsos2020agora}). 

To further improve data security, more advanced cryptographic techniques like homomorphic and functional encryption have been utilized to generate analytics over the raw data for consumers to purchase without revealing the data themselves~\cite{duan2019aggregating,niu2018unlocking,niu2018achieving,koutsos2020agora}. However, we note that these approaches are limited in the following three aspects: 1) data owners upload the encrypted raw data on the blockchain, which leads to permanent loss of the data ownership to any adversarial party with the decryption key; 2) the available analytics are limited to simple linear combinations; 3) they still require a (trusted or untrusted) third party other than the data owner and consumer acting like a broker or service provider to maintain the utility and security of trading session. 

% A key consideration of developing such data markets is privacy and security. Specifically, the data owners would not like to have their private data revealed during the trading process, and would like to be properly compensated for their data contributions; the data consumers would like to purchase data that is faithfully collected or generated.

In this paper, our goal is to build a secure, robust, and broker-free data market for general machine learning applications. Particularly, a model owner would like to crowdsource training data from interested data owners through the data market for improving the quality of its ML models (e.g., a deep neural network for image classification). Moreover, we enforce the following privacy and security requirements:
\begin{itemize}[leftmargin=*]
    \item \emph{Model privacy}: the ML model is only known at the model owner and not revealed to other parties;
    \item \emph{Data privacy}: model owner learns nothing about data owners' private other than the learnt model;
    \item \emph{Byzantine resistance}: 1) robust to malicious data owners who intentionally provide incorrect data, and 2) robust to malicious model owner who tries to evade paying for the model training.
\end{itemize}

We propose a novel blockchain-based data market named \scheme, which is the first implementation of an \ethe smart contract~\cite{ETH} that simultaneously satisfies all the above security requirements. During a trading session, the model owner deploys a smart contract with the encrypted initial ML model, then interested data owners retrieve the published model, compute locally the gradients using their private data, and upload the gradients back to the contract. During this process, the data owners hide their local gradients with pair-wise masks generated according to the secure aggregation protocol~\cite{bonawitz2017practical} to further protect data leakage. Moreover, \scheme implements the multi-Krum algorithm~\cite{blanchard2017machine,blanchard2017byzantine} to remove faulty computation results from malicious data owners. Finally, the model owner decrypts the aggregated gradients from many data owners with its private key, and uses the results to update its model. The training reward is provided by the model owner when deploying the contract, and is automatically distributed to honest data owners by the contract, preventing malicious model owners from evading payments after obtaining the trained model.

We implement an \ethe smart contract \contract and the off-chain application of the proposed \scheme data market. We conduct extensive experiments to measure the gas cost and the execution time of \contract under various combinations of system parameters. 
% We conduct evaluation by deploy smart contracts on the Ethereum chain and generate multiple data owners instances. They greedily register with active contract to upload their results until the results are incorporated in the ﬁnal aggregation. 
Within the considered parameter range, all interaction processes between the data owner and the contract are completed within 0.8s, and all interaction processes between the model owner and the contract are completed within 18s. This demonstrates the high efficiency and feasibility of the proposed \scheme data market. %Finally, $\scheme$ achieves high efficiency and feasibility, while realizing the innovation of Secure Aggregation running on blockchain.

%\subsection*{Related works}

{\bf Secure data markets.} While traditional data markets are implemented as an intermediate service platform that helps to enforce desirable rules about data privacy, data ownership, and data usage, this requires full trust on the platform and leaves the platform the single point of failure in maintaining these properties. To resolve this issue, implementing the data market service over decentralized systems like blockchains has been recently proposed~\cite{ozyilmaz2018idmob,ramachandran2018towards,banerjee2018blockchain,duan2019aggregating,koutsos2020agora}. In these implementations, encrypted data are uploaded to the blockchain, on which a smart contract with funding deposit from the consumer is executed automatically, guaranteeing the atomicity of the payment. To further enhance the data privacy and robustness to malicious behaviors, more advanced techniques like homomorphic encryption, functional encryption, and differential privacy have been utilized to generate simple analytics over the raw data for sale without revealing the individual data points~\cite{duan2019aggregating,niu2018unlocking,koutsos2020agora}, and zero-knowledge proofs and trusted hardware like Intel SGX have been used to guarantee the correctness of the computations~\cite{duan2019aggregating,niu2018achieving,koutsos2020agora}. 

{\bf Federated learning on blockchains.} Federated learning (FL)~\cite{mcmahan2017communication} has recently been proposed as a privacy-preserving framework for distributed ML where a set of clients, instead directly uploading their private data to the cloud, upload the gradients computed from the data, which are aggregated at a cloud server to update a global model. In addition, techniques of masking local gradients like secure aggregation~\cite{bonawitz2017practical,bell2020secure,so2021turbo} and differential privacy~\cite{geyer2017differentially,wei2020federated} have been developed for FL to further protect potential data leakage.

Recently, it has been proposed to execute FL tasks on blockchains to combat server corruption and facilitate a more fair and transparent reward distribution (see, e.g.,~\cite{zhao2020privacy,liu2020fedcoin,kim2019blockchained,shayan2020biscotti,ma2020federated}). In~\cite{zhao2020privacy}, a FL on blockchain system is designed for the smart appliance manufactures to learn a ML model from customers' data. Differential privacy techniques are applied on the clients' extracted features to protect data privacy from the computed gradients that are uploaded on the blockchain. A reputation-based incentive mechanism is designed to reward contributing customers and punish malicious ones. However, one weakness of the design in~\cite{zhao2020privacy} is that the initial model of the manufacturer is revealed to public, which may not be desirable for the model owner, especially for an iterative training session where the initial model for an iteration is learnt using customers' data from previous iterations. Also, \cite{zhao2020privacy} does not provide a blockchain implementation of their design. In~\cite{liu2020fedcoin}, a P2P payment blockchain protocol is designed to compute and distribute the profit in a FL session, based on evaluations of Shapley values. The protocol in~\cite{liu2020fedcoin} is fundamentally different from the proposed \scheme data market as FL and reward distribution are performed on two separate systems in~\cite{liu2020fedcoin}.  

In another recent work~\cite{lyu2020towards}, another federated learning framework over blockchain named FPPDL was proposed to facilitate fair and privacy-preserving machine learning. While both FPPDL and the proposed \scheme data market have data owners and model owners respectively upload and download encrypted gradients via blockchain transactions,
they differ drastically in the implementations of underlying blokchain systems. In FPPDL, a data owner is co-located with a blockchain miner such that a learning participant has to perform local training and block verification. As a participant needs permission to join the system, FPPDL is restricted to permission blockchains. However, \scheme does not have such restriction as the entire data market is implemented as a smart contract on top of a existing blockchain such that the data owners and the block miners operate independently. This allows \scheme to be implemented on permissionless public blockchains like \ethe where data owners can be rewarded with the corresponding cryptocurrencies.

==> verifyAgg.tex <==

\section{Multi-server Publicly Verifiable Gradient Validation and Aggregation of \scheme}

To speed up the contract execution, and reduce the fees for on-chain transaction verification, \scheme delegates the storage and processing of \drs' gradients to a set of off-chain servers. The servers collectively verify the validity of each \dr's gradient, by evaluating a validation predicate $\texttt{Valid}(\cdot)$ specified by the \mr. Then, the validated gradients are aggregated to update \mr's model. To protect the privacy of \drs' local data, and verify the integrity of servers' computations on-chain, we design the gradient validation and aggregation process of \scheme based on a publicly verifiable computation scheme in~\cite{zhang2022multi}, which we describe in the following.

\noindent {\bf Step 1: Secret sharing of gradient.} Each \dr creates a share of its secret gradient $\vct{g} \in \mathbb{F}^m$ 


\noindent {\bf Step 2: Publicly verifiable gradient validation.}


\noindent {\bf Step 3: Publicly verifiable gradient aggregation.}

